Gerrymandering Planar Graphs

We study the computational complexity of the map redistricting problem (gerrymandering). Mathematically, the electoral district designer (gerrymanderer) attempts to partition a weighted graph into $k$ connected components (districts) such that its candidate (party) wins as many districts as possible. Prior work has principally concerned the special cases where the graph is a path or a tree. Our focus concerns the realistic case where the graph is planar. We prove that the gerrymandering problem is solvable in polynomial time in $\lambda$-outerplanar graphs, when the number of candidates and $\lambda$ are constants and the vertex weights (voting weights) are polynomially bounded. In contrast, the problem is NP-complete in general planar graphs even with just two candidates. This motivates the study of approximation algorithms for gerrymandering planar graphs. However, when the number of candidates is large, we prove it is hard to distinguish between instances where the gerrymanderer cannot win a single district and instances where the gerrymanderer can win at least one district. This immediately implies that the redistricting problem is inapproximable in polynomial time in planar graphs, unless P=NP. This conclusion appears terminal for the design of good approximation algorithms -- but it is not. The inapproximability bound can be circumvented as it only applies when the maximum number of districts the gerrymanderer can win is extremely small, say one. Indeed, for a fixed number of candidates, our main result is that there is a constant factor approximation algorithm for redistricting unweighted planar graphs, provided the optimal value is a large enough constant.

==> appendicies.tex <==

\section{A Dynamic Program for Graphs of Bounded Treewidth}\label{sec:missingDPproof}


In this appendix, we present a dynamic program for the gerrymandering problem in graphs of bounded treewidth. In particular, we prove Theorem~\ref{thm:boundedTW}.

\boundedTW*
We begin with the necessary definitions concerning treewidth.
\begin{definition}\label{def:treewidth}
A \emph{tree decomposition} of a graph $G$ is a pair $(T,\beta)$ of a tree $T$
and $\beta:V(T) \rightarrow 2^{V(G)}$, 
such that:
\begin{itemize}
    \item $\bigcup\limits_{v \in V(T)} \beta(v) = V(G)$, and
    \item\label{item:twedge} for any edge $\{\rho,\rho'\} \in E(G)$ there exists a node $v \in V(T)$ such that $\rho,\rho' \in \beta(v)$, and
    \item\label{item:twconnected} for any vertex $\rho \in V(G)$, the subgraph of $T$ induced by the set $T_\rho = \{v\in V(T): \rho\in\beta(v)\}$ is a tree.
\end{itemize}
The {\em width} of $(T,\beta)$ is $\max\limits_{v\in V(T)}\{|\beta(v)|\}-1$. The {\em treewidth} of $G$ is the minimum width of a tree decomposition of $G$.
\end{definition}
For $v \in V(T)$, we say that $\beta(v)$ is the \emph{bag} of $v$. Let $\tw(G)$ denote the treewidth of $G$. Now if $(T,\beta)$ denotes a tree decomposition of $G$, we can transform in polynomial time $(T,\beta)$ into a {\em nice} tree decomposition of the same width~\cite{DBLP:journals/siamcomp/Bodlaender96} and with $O(n)$ nodes. A nice tree decomposition is one where $T$ is a binary tree, a node with two children has the same bag as its children, and any other node either has an empty bag or a bag that differs by exactly one vertex from the bag of its child. Moreover, the bag of the root, denoted by $r$, is empty. 

Let $G = (V, E)$ be a weighted graph with weight function $wt: V(G) \rightarrow \mathbb{N}$, and let $T$ be a nice tree decomposition of $G$ with treewidth $\tw(G)$. For a node $X$ of the tree decomposition, a \textit{configuration} of $X$ is a tuple $(\kappa,\omega,P,\gamma)$. A configuration of $X$ is \textit{valid} if there exists a partition $\mathbf{P}$ of the subgraph induced by the subtree rooted at $X$ such that:
\begin{itemize}
    \item $\kappa\in \{1,\dots,k\}$ is the number of districts in $\mathbf{P}$
    \item $\omega \in \{1,\dots,\kappa\}$ is the number of districts won by candidate $1$ (the blue candidate).
    \item $P$ is a partition of $\beta(X)$, and two vertices in $\beta(X)$ are in the same district in $P$ if and only if they are in the same district in $\mathbf{P}$.
    \item $\gamma: P \times \{1,\dots,c\}  \rightarrow \{1,\dots,\sum\limits_{v\in V} wt(v)\}$ is a function; $\gamma(D,i)$ indicates for any district $D$ of $X$ and any color $i\in \{1,\dots,c\}$ the number of votes received by candidate $i$ in the district $\mathbf{D}\in \mathbf{P}$ such that $D\subset \mathbf{D}$.
\end{itemize}
In that case we say that $(\kappa,\omega,P,\gamma)$ is \textit{coherent} with $\mathbf{P}$.

The dynamic program calculates the function $\varphi$, which takes a node $X$ of the tree decomposition as input and generates a list of all valid configurations. We employ a bottom-up approach, whereby the dynamic program first processes the leaf nodes of the tree decomposition $T$, and then computes $\varphi({X})$ for all nodes in $T$.

The initialization step is straightforward since all leaf nodes are empty. The updating steps vary depending on the type of node, and the following programs provide explanations for each type.\\

\noindent\textbf{Join Node:} Suppose $X$ is a join node with children $L$ and $R$, and we have already computed $\varphi(L)$ and $\varphi(R)$. Let $(\kappa_L,\omega_L,P_L,\gamma_L)$ and $(\kappa_R,\omega_R,P_R,\gamma_R)$ be two valid configurations of $L$ and $R$, respectively. Then there exist two partitions $\mathbf{P}_L$ and $\mathbf{P}_R$ of the subgraphs induced by the subtrees rooted in $L$ and $R$, respectively, such that $\mathbf{P}_L$ is coherent with $(\kappa_L,\omega_L,P_L,\gamma_L)$ and $\mathbf{P}_R$ is coherent with $(\kappa_R,\omega_R,P_R,\gamma_R)$.

We can merge $\mathbf{P}_L$ and $\mathbf{P}_R$ into a new partition $\mathbf{P}$ if and only if $P_L = P_R$. In this case, the resulting configuration $(\kappa,\omega,P,\gamma)$ coherent with $\mathbf{P}$ is:
\begin{itemize}
    \item We have $P= P_L = P_R$.
    \item A district is either only in $\mathbf{P}_L$, only in $\mathbf{P}_R$ or it intersects $\beta(X)$. Therefore $\kappa = \kappa_L + \kappa_R - |P|$. If $\kappa > k$, the configuration is not valid.
    \item Similarly for any district $D$ of $P$ and any color $i$, we have \[\gamma(D,i) = \gamma_L(D,i) + \gamma_R(D,i) - \sum\limits_{v\in D:v\text{ colored }i} wt(v).\]
    \begin{sloppypar}
    \item To compute the number of winning districts, we first define $W_L$, $W_R$ and $W$ as the sets of districts in $P$ that are won by blue in the corresponding districts of $\mathbf{P}_L$, $\mathbf{P}_R$ and $\mathbf{P}$ respectively. Specifically, $W_L := \{D\in P: \gamma_L(D,1)>\gamma_L(D,i) \text{ for any color }i \neq 1\}$, $W_R := \{D\in P: \gamma_R(D,1)>\gamma_R(D,i) \text{ for any color }i \neq 1\}$ and $W := \{D\in P: \gamma(D,1)>\gamma(D,i) \text{ for any color }i \neq 1\}$. Next, we compute the number of winning districts in $\mathbf{P}_L$ and $\mathbf{P}_R$ that do not intersect $\beta(X)$. Specifically, the number of winning districts in $\mathbf{P}_L$ is $\omega_L - |W_L|$, and the number of winning districts in $\mathbf{P}_R$ is $\omega_R - |W_R|$. Finally, we compute the number of winning districts in the merged partition $\mathbf{P}$: $\omega = \omega_R + \omega_L - |W_L| - |W_R| + |W|$.
    \end{sloppypar}
\end{itemize}

To compute $\varphi(X)$ from $\varphi(L)$ and $\varphi(R)$, we need to consider all possible pairs of $(\kappa_L,\omega_L,P_L,\gamma_L) \in \varphi(L) $ and $(\kappa_R,\omega_R,P_R,\gamma_R)\in \varphi(R)$. For each pair, we check if a valid configuration exists. If so, we add it to a list and remove duplicate entries.\\

\noindent\textbf{Forget Node:} Assume $X$ is a forget node with a child $Y$ such that $\beta(X) = \beta(Y)\setminus {v}$.  Let $(\kappa_Y,\omega_Y, P_Y, \gamma_Y)$ be a valid configuration for $Y$ coherent with a partition $\mathbf{P}$ of the subgraph induced by the subtree rooted in $Y$. Note that the subtree rooted at $X$ induces the same subgraph as the subtree rooted at $Y$. There are two cases to consider:

Case 1: ${v}\in P_Y$ is a singleton district. In this case, the configuration $(\kappa,\omega,P,\gamma)$ of $X$ coherent with $\mathbf{P}$ is given by $\kappa = \kappa_Y$, $\omega = \omega_Y$, $P = P_Y\setminus{{y}} $, and $\gamma = \gamma_Y|P$ where $\gamma_Y|P$ is defined to be the same as $\gamma_Y$ for each district in $P$.

Case 2: $v \in D$ for some district $D\in P_Y$. Then, the configuration coherent with $\mathbf{P}$ is given by:
$\kappa = \kappa_Y$, $\omega = \omega_Y$, $P$ is obtained from $P_Y$ by removing ${v}$ from the district $D$, so $P = (P_Y\setminus {D}) \cup ({D \setminus{v}})$. We have $\gamma(D',i) = \gamma_Y(D',i)$ for any color $i$ and district $D \neq D \setminus{v}$, and $\gamma(D\setminus{v},i) = \gamma_Y(D,i)$ for any color $i$.\\

\noindent\textbf{Introduce Node:} Assume $X$ is an introduce node with child $Y$ such that $\beta(X) = \beta(Y) \cup \{v\}$. Let $(\kappa_Y,\omega_Y, P_Y, \gamma_Y)$ be a valid configuration of $Y$ coherent with a partition $\mathbf{P}$ of the subgraph induced by the subtree rooted in $Y$. Note that then the subgraph induced by the subtree rooted at $X$ is the same as the one rooted at $Y$ with an extra vertex $v$. We need to compute all possible configurations $(\kappa, \omega, P, \gamma)$ obtained by extending $\mathbf{P}$. Define $N(v):=\{u \in \beta(X):(u,v)\in E\}$, the neighborhood of $v$ in the graph induced by $\beta(X)$. For any subset $S\subseteq N(v)$ ($S$ can be empty), the districts induced by the vertices in $S$ can be connected using $v$ and merged. In that case the configuration $(\kappa, \omega, P, \gamma)$ can be computed from $(\kappa_Y,\omega_Y, P_Y, \gamma_Y)$. First we define the set $\Delta_S := \{D\in P_Y : D \cap S \neq \emptyset \}$, the set of districts of $P_Y$ intersecting $S$.
\begin{itemize}
\item The new partition is obtained by merging districts in $\Delta_S$ with $\{v\}$: $$P = P_Y\setminus \Delta_S \bigcup \left\{ (\bigcup\limits_{D\in\Delta_S} D) \cup \{v\}\right\}$$
\item The number of districts is $\kappa = \kappa_Y - |\Delta_S|+1$.
\item For any color and any district $D\in P_Y$ not in $\Delta_S$, we have $\gamma(D,i) = \gamma_Y(D,i).$ For the district $(\bigcup\limits_{D\in\Delta_S} D) \cup \{v\}$, we have \[\gamma((\bigcup\limits_{D\in\Delta_S} D) \cup \{v\},i) = \sum \limits_{D\in \Delta_S} \gamma_Y(D,i) + \begin{cases} wt(v) & \text{ if } v\text{ colored } i \\
0 & \text{ otherwise.}\end{cases}\]
\item To compute the updated number of winning districts, we need to first remove those winning districts in $\Delta_S$ and recompute the winning status after merging $\Delta_S$ with $\{v\}$. The number of winning districts in $\Delta_S$ is given by $|\{D\in \Delta_S: \gamma_Y(D,1)>\gamma_Y(D,i), \forall i \not=1\}|$. The new merged district $(\bigcup\limits_{D\in\Delta_S} D) \cup \{v\}$ is winning if \[\gamma((\bigcup\limits_{D\in\Delta_S} D) \cup \{v\},1) > \gamma((\bigcup\limits_{D\in\Delta_S} D) \cup \{v\},i), \forall i\not=1.\] Concretely:
\begin{multline*}
    \omega = \omega_Y - |\{D\in \Delta_S: \gamma_Y(D,1)>\gamma_Y(D,i), \forall i \not=1\}| \\+ \begin{cases}
    1, &\text{if } \gamma((\bigcup\limits_{D\in\Delta_S} D) \cup \{v\},1) > \gamma((\bigcup\limits_{D\in\Delta_S} D) \cup \{v\},i), \forall i\not=1\\
    0, &\text{otherwise. }
\end{cases}
\end{multline*}
\end{itemize}


Finally, at the root node, the largest $\omega$ is the maximum number of winning districts for the target candidate $1$ satisfying the constraint that the total number of districts is at most~$k$.\\

\noindent\textbf{Time Complexity:} Let $S$ be the number of possible configurations $(\kappa, \omega, P, \gamma)$ of a single bag. For each configuration, there are $k$ possible values for $\kappa$ and $\omega$; the number of partitions is upper bounded by $\tw^{\tw}$; and the number of functions $\gamma: P \cdot \{1,\dots, c\} \rightarrow \{1,\dots, \sum\limits_{v\in V} wt(v)\}$ is at most $(\sum\limits_{v\in V} wt(v))^{c\cdot\tw}$. So $S \le k^2 \cdot \tw^{\tw} \cdot (\sum\limits_{v\in V} wt(v))^{c\cdot\tw} \le n^{2+tw} \cdot (\sum\limits_{v\in V} wt(v))^{c\cdot\tw}$. We now bound the time to compute all the valid configurations of a node, given the valid configurations of its child nodes. 

For a join node, the algorithm will consider all pairs of configurations of its child nodes and there are at most $S^2$ such pairs. For each pair of configuration, it takes constant time to compute $P$ and $\kappa$; and at most $O(c\cdot\tw) = O(n^2)$ time to compute both $\gamma$ and $\omega$, so the running time in this case is bounded by $O(S^2 \cdot n^2)$.  For a forget node, there is only one child with $S$ different configurations to consider. Fixing a configuration, it takes constant time to compute all parameters but $\gamma$, which takes time $O(c\cdot\tw) = O(n^2)$. For a introduce node, there is also only one child. Fixing a configuration, the algorithm needs to compute all possible partitions. The number of possible choice is bounded by $(\tw+1)$. The running time for computing $\omega$ and $\gamma$ is at most $O(c\cdot\tw) = O(n^2)$ each. It follows that the time complexity for computing a single node is dominated by the join nodes. Therefore the total running time is bounded by $O(n)\cdot O(S^2 \cdot n^2) = O(n^{2\tw+7}\cdot (\sum\limits_{v\in V} wt(v))^{2c\cdot\tw})$.\\

This completes the proof of Theorem~\ref{thm:boundedTW}.


\section{Hardness Proofs}\label{sec:missinghardnessproof}

In this appendix, we give the prove our hardness result for gerrymandering in general graphs.

\hardness*
\begin{proof}
    Let $G$ be a graph with $|V(G)|=n$. We derive an auxiliary graph $H$ from $G$ such that there exists an  independent set of size $w$ in $G$ if and only if there exists a $(n,w)$-partition of $H$. The construction of $H$, illustrated in
    Figure~\ref{fig:hard-general}, is as follows:
    \begin{itemize}
        \item For each vertex $v \in V(G)$, there is a blue vertex $b^v\in V(H)$.
        \item For each edge $e=(u,v) \in E(G)$, we create $2n$ red vertices $r^e_i\in V(H)$ for $i = 1,\dots,2n$. Each such red vertex has edges in $E(H)$ to both $b_v$ and $b_u$.
    \end{itemize}
\begin{figure}[h]
\centerline{\includegraphics[width = 8cm]{IndependentSetReduction.png}}
\caption{Construction of $H$ in the proof of Lemma~\ref{lem:hardness}}\label{fig:hard-general}
\end{figure}


Now consider the gerrymandering problem in $H$ with $n$ districts. The first task is to prove that in a valid decomposition of $H$ into $n$ connected districts any winning district must be a blue singleton vertex. Suppose we have a winning district $D_i$ that is not a blue singleton. Then $D_i$ must contain at least two blue vertices. 
Furthermore, by the connectivity requirement, there must be vertices $b_u, b_v \in D_i$ such that the edge $e = (u,v)\in E(G)$. Because $H$ only has $n$ blue vertices, $D_i$ can have at most $n-1$ red vertices. Consequently, there must be at 
least $n+1$ red vertices of the form $r_j^e$, for some $j \in \{ 1,\dots,2n\}$, which are {\bf not} in $D_i$. 
But these red vertices must each then form a singleton district. Thus there are at least $n+1$ districts, a contradiction.

We will now demonstrate that the set $\{b^v: v\in S\}$ is a collection of blue winning singleton-districts in $H$ if and only if $S$ is an independent set in $G$. First, assume $S$ is an independent set in $G$. We create a partition of $V(H)$ such that $V(H) = \bigcup_{v\in V(G)} D_v$ and start with $D_v = {b_v}$, for each $v\in V(G)$. 
Now since $S$ is an independent set, $V(G)\setminus S$ is a vertex cover in $G$.
Thus, for every $e\in E(G)$, there exists $v_e \in V(G)\setminus S$ which is an endpoint of $e$. We add all vertices of the form $r^e_i$ to $D_{v_e}$. Observe this induces a partition of $H$ into $n$ connected districts where $\{b^v: v\in S\}$ in $H$ are a collection of blue-winning singleton districts.
Second, assume that $\{b^v: v\in S\}$ is a collection of blue-winning singleton districts in $H$. Assume for a contradiction 
that $S$ is not an independent set in $G$. Then there exists an edge $(u,v)\in E(G)$ where $\{u, v\}\subseteq S$. This implies all the vertices $r_j^e$, for $j \in \{ 1,\dots,2n\}$, must be singleton districts, contradicting the fact there are $n$ districts. 
 \end{proof}

\hardgeneral*

\begin{proof}
According to the result of Zuckerman \cite{Z2006}, the maximum independent set (or clique) problem cannot be approximated within a factor of $n^{1-\epsilon}$ unless $P = NP$, strengthening the work of H\r{a}stad~\cite{Hstad1999}. The theorem then follows from Lemma~\ref{lem:hardness}, because the number of vertices of the graph $H$ used in the proof is bounded by $|V(G)| + 2\cdot |V(G)| \cdot |E(G)|  \leq |V(G)|^3$.
 \end{proof}






% \section{PTAS Proof}\label{sec:missingPTASproof}

% Finally, in this appendix we prove there is a PTAS for the singleton winning district problem in
% planar graphs. 
% \ptas*

% The first step in our PTAS is a preprocessing step 
% based upon Baker's classical partitioning technique
% for planar graphs\cite{Baker1994}.
% \begin{algorithm}[H]
% \caption{Preprocessing via Baker's Technique}\label{alg:ptas}
% \begin{algorithmic}[1]
% \State{\textbf{Input:} A planar graph $G$ with vertices colored blue or red, an integer $\lambda$, and an integer $j \in \{0,\lambda-1\}$}
% \State{Fix a planar embedding $P$ of $G$}
% \State{Set $i = 1$}
% \While{$P$ non-empty}
% \State{Set $L_i$ to be the vertices on the outer face of $P$}
% \If{$i \equiv j \mod \lambda$}
% \State{color every vertex $u \in L_i$ red}
% \State{Contract all edges $(u,v)$ with  $u,v \in L_i$}
% \EndIf
% \State{Delete $L_i$ from $P$}
% \State{Set $i = i+1$}
% \EndWhile
% \State{\textbf{Output:} The resultant graph $G_{\lambda,j}$}
% \end{algorithmic}
% \end{algorithm}

% So, for a fixed $\lambda$, the preprocessing step creates a set of graphs
% $\{G_{\lambda,0}, G_{\lambda,1}, \dots, G_{\lambda,\lambda-1}\}$.
% We claim that at least one of these graphs has a solution almost as large
% as the optimal solution in the original graph $G$.
% This is guaranteed by the next lemma.
% \begin{lemma}\label{lem:preprocess}
% With only singleton winning districts the following hold:
% \begin{enumerate}
%     \item Any $(k,w)$-partition of $G_{\lambda,j}$ induces a $(k,w)$-partition of $G$, for all $k,w$. \label{preprocess1}
%     \item For any $\lambda$, there exists $j \in \{0,\lambda-1\}$ and $w^*\geq w_{OPT} \cdot \frac{\lambda-1}{\lambda}$ such that there exists a $(k,w^*)$-partition of $G_{\lambda,j}$. \label{preprocess2}
% \end{enumerate}
% \end{lemma}
% \begin{proof}
% Observe that \ref{preprocess1}. holds trivially by construction of the preprocessing algorithm.
% So consider \ref{preprocess2}. Let $\lambda$ be an integer and take a $(k,w_{OPT})$-partition of $G$
% for the singleton winning district gerrymandering problem. Denote by $B_W$ the set of winning blue vertices. Then there exists $j$ such that $|B_W \cap \bigcup_{i \equiv j \mod{\lambda}}L_i| \leq \frac{1}{\lambda} \cdot w_{OPT}$. Let $w^*:= |B_W \setminus{ \bigcup_{i \equiv j \mod{\lambda}}L_i}|$, the partition in $G$ then induces a $(k,w^*)$-partition in $G_{\lambda,j}$, as required.
%  \end{proof}

% Lemma~\ref{lem:preprocess} implies that by solving the 
% singleton winning district gerrymandering problem in the appropriate 
% graph $G_{\lambda,j}$ may produce a PTAS for the original graph $G$.
% But how can we solve the problem in $G_{\lambda,j}$.
% The key is to demonstrate that each graph $G_{\lambda,j}$ has bounded tree-width. 

% \begin{lemma}\label{lem:bounded-treewidth}
%  Each graph $G_{\lambda,j}$ has treewidth at most $3\lambda-1$. 
% \end{lemma}
% \begin{proof}
% The proof will use the that a $\lambda$-outerplanar has treewidth at most $3\lambda-1$, as shown by Bodlaender~\cite{Bodlaender1998}. 
% Unfortunately we cannot apply Bodlaender's result directly to $G_{\lambda,j}$ because it may have an unbounded outerplanarity index.
% However, we can still utilize the result.

% Specifically, we prove the lemma by induction on the size of $S=\{i:L_i \neq \emptyset, \, i \equiv j\mod\lambda\}$. For the base case, if $|S|=0$,
% then the graph $G_{\lambda,j}$ has at most $\lambda$ layers so
% its is $\lambda$-outerplanar and thus has treewidth at most $3\lambda-1$.

% For the induction step, consider $\bigcup_{i\leq j}L_i$ and 
% $G_{\lambda,j}\setminus\bigcup_{i<j}L_i$. The former has treewidth
% at most $3\lambda-1$ because it is $\lambda$-outerplanar. The latter 
% has treewidth at most $3\lambda-1$ by the induction hypothesis.
% To show that $G_{\lambda,j}$ has has treewidth at most $3\lambda-1$, 
% observe that the outer face of a connected planar graph is itself connected.
% Now consider a contraction step in the preprocessing algorithm.
% This implies that each vertex in $L_j$ that remains after the contraction step must correspond to the outer face of a connected component in the graph $G\setminus\bigcup_{l<i}L_l$. 
% Now let $T$ be tree decomposition $\bigcup_{i\leq j}L_i$ after the vertices in $L_j$ have been contracted.
% Further, for each vertex $x\in L_j$, let $T_x$ be a tree decomposition of the corresponding connected component of $G_{\lambda,j}\setminus\bigcup_{i<j}L_i$. We may root each $T_x$ at a node containing $x$ in its bag. We can then merge $T$ with $T_x$ by connecting the root of $T_x$ to any node of $T$ that contains $x$ in its bag. We do this for each $x\in L_j$. This gives a tree
% decomposition of width $3\lambda-1$. To see that the resultant tree decomposition is valid observe that the paths in $G_{\lambda,j}$ connecting a vertex of $T$ to a vertex of $T_x$ must necessarily pass through the vertex $x$, which corresponds to the outer face of the connected component induced by the verticess in $T_x$.
%  \end{proof}


% \begin{proof}[Proof of Theorem~\ref{thm:ptas}]
% Let $\epsilon > 0$. We choose $\lambda = \lceil \frac{1+\epsilon}{\epsilon} \rceil$. For each $j$, we run the dynamic programming algorithm described in Section~\ref{section:boundedTW} on $G_{\lambda,j}$. Since $G_{\lambda,j}$ has bounded treewidth by Lemma~\ref{lem:bounded-treewidth} and Theorem~\ref{thm:boundedTW}, this can be done in polynomial time. Now using Lemma~\ref{lem:preprocess}, there exists a $j$ such that the algorithm produces a $(k,w\cdot \frac{\lambda-1}{\lambda})$-partition of $G_{\lambda,j}$ inducing a $(k,w\cdot \frac{\lambda-1}{\lambda})$-partition of $G$. We picked $\lambda$ such that $\frac{\lambda-1}{\lambda} \geq \frac{1}{1+\epsilon}$ so we get a $(1+\epsilon)$-approximation. Since this holds for any $\epsilon > 0$, we have a polynomial-time approximation scheme.
%  \end{proof}


